Smarter Features, Simpler Learning?

Earlier work on machine learning for automated reasoning mostly relied on simple, syntactic features combined with sophisticated learning techniques. Using ideas adopted in the software verification community, we propose the investigation of more complex, structural features to learn from. These may be exploited to either learn beneficial strategies for tools, or build a portfolio solver that chooses the most suitable tool for a given problem. We present some ideas for features of term rewrite systems and theorem proving problems.

==> eptcsdata.tex <==
\providecommand{\firstpage}{25}
\providecommand{\publicationstatus}{M. Suda, S. Winkler (Eds.): Second International Workshop\\
on Automated Reasoning: Challenges, Applications,\\
Directions, Exemplary Achievements (ARCADE 2019)\\
EPTCS 311, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.311.4}{10.4204/EPTCS.311.4}}
\pdfoutput=1

